Maximum Matching in Two, Three, and a Few More Passes Over Graph Streams

We consider the maximum matching problem in the semi-streaming model formalized by Feigenbaum, Kannan, McGregor, Suri, and Zhang that is inspired by giant graphs of today. As our main result, we give a two-pass $(1/2 + 1/16)$-approximation algorithm for triangle-free graphs and a two-pass $(1/2 + 1/32)$-approximation algorithm for general graphs; these improve the approximation ratios of $1/2 + 1/52$ for bipartite graphs and $1/2 + 1/140$ for general graphs by Konrad, Magniez, and Mathieu. In three passes, we achieve approximation ratios of $1/2 + 1/10$ for triangle-free graphs and $1/2 + 1/19.753$ for general graphs. We also give a multi-pass algorithm where we bound the number of passes precisely---we give a $(2/3 -\varepsilon)$-approximation algorithm that uses $2/(3\varepsilon)$ passes for triangle-free graphs and $4/(3\varepsilon)$ passes for general graphs. Our algorithms are simple and combinatorial, use $O(n \log n)$ space, and have $O(1)$ update time per edge. For general graphs, our multi-pass algorithm improves the best known deterministic algorithms in terms of the number of passes: --Ahn and Guha give a $(2/3 - \varepsilon)$-approximation algorithm that uses $O(\log(1/\varepsilon)/\varepsilon^2)$ passes, whereas our $(2/3 - \varepsilon)$-approximation algorithm uses $4/(3\varepsilon)$ passes; --they also give a $(1-\varepsilon)$-approximation algorithm that uses $O(\log n \cdot \mathrm{poly}(1/\varepsilon))$ passes, where $n$ is the number of vertices of the input graph; although our algorithm is $(2/3 - \varepsilon)$-approximation, our number of passes do not depend on $n$. Earlier multi-pass algorithms either have a large constant inside big-$O$ notation for the number of passes or the constant cannot be determined due to the involved analysis, so our multi-pass algorithm should use much fewer passes for approximation ratios bounded slightly below $2/3$.

==> mcm_sumedh2.tex <==
\section{Further Improved Two Pass Algorithm}\label{sec:2pimp3}
The Algorithm described in this Section has a minor modification
over~\Cref{alg:2pimp2}. When a new edge $xy$ forms a length-$3$ augmenting path
with edges $yv\in M_0$ and $ vb\in S$, we augment only if the number of edges
incident on $x$ in $S$ is strictly less than $\lambdaU$. Using this minor
modification, we are able to reduce the number of partially good edges that are
charged to a good edge, thereby improving the approximation
ratio. \Cref{alg:2pimp3} gives a formal description.
\begin{algorithm}[!ht]
  \caption{Further improved two-pass algorithm\label{alg:2pimp3}: input graph
    $G$}
  \begin{algorithmic}[1]
    \State In the first pass, find a maximal matching $M_0$.
    \If{$G$ is triangle-free}
    \State Return Best of \textproc{Improve-Matching}$(M_0,2,1)$ and
    \textproc{Improve-Matching}$(M_0,3,1)$ 
    \Else
    \State Return \textproc{Improve-Matching}$(M_0,4,2)$
    \EndIf
    % Short version
    % \State If $G$ is triangle-free, then $\lambdaU \gets 2, \lambdaM \gets 1$,
    % else $\lambdaU \gets 4, \lambdaM \gets 2$.
    % \State Return \textproc{Improve-Matching}$(M_0,\lambdaU,\lambdaM)$

    \Function{Improve-Matching}{$M_0, \lambdaU, \lambdaM$}
    \label{alg:2pimp3:fimpm}
    \State  $M\gets M_0$, $S\gets\emptyset$, $I\gets \emptyset$ and
    $I_B\gets \emptyset$
    \ForAll{edge $xy$ in the stream} \label{line:alg:2pimp3:4}
    % Short version
    % \If{($x \text{ or } y\in I \cup I_B)$ or ($x\in V(M_0)$ and
    % $y\in V(M_0)$)}\label{line:9}
    % \State Continue, i.e., ignore $xy$.
    \If{$x \text{ or } y\in I \cup I_B$}\label{line3:9}
    \State Continue, i.e., ignore $xy$.
    \ElsIf{$x\in V(M_0)$ and $y\in V(M_0)$}
    \State Continue, i.e., ignore $xy$.
    \ElsIf{there exist $v$ and $b$ such that $\deg_S(x) <\lambdaU$, $yv \in
      M_0$, and $vb \in S$} 
    \State
    $M\gets M\setminus \{yv\} \cup \{xy,vb\}$ \label{line3:c3aug}
    \Comment{a $3$-augmentation}
    \Statex \hskip\algorithmicindent \hskip\algorithmicindent
    \hskip\algorithmicindent 
    Let
    $I_x\gets\{u_x\,,v_x: xu_x\in S \text{ and } u_xv_x\in M_0 \}$.
    \Statex \hskip\algorithmicindent \hskip\algorithmicindent
    \hskip\algorithmicindent 
    Let
    $I_b\gets\{u_b\,,v_b: u_bv_b\in M_0 \text{ and } v_bb\in S \}$. 
    \State Then $I\gets I\cup \{x,y,v,b\}$ and $I_B\gets I_B \cup I_x \cup I_b$.
    \Else
    \Statex \hskip\algorithmicindent \hskip\algorithmicindent
    \hskip\algorithmicindent 
    Without loss of generality, assume that $x\in V\setminus V(M_0)$ and $y\in
    V(M_0)$.
    \If{$\deg_S(x) <\lambdaU$ and $\deg_S(y)<\lambdaM$}
    \Comment{See~\Cref{fig:2pimp2}.}
    % Short version \Comment{See~\Cref{fig:2pimp2} in Appendix.}
    \State $S\gets S\cup \{xy\}$
    \Comment{\textbf{Note:} Once an edge is added to $S$, it is never removed
      from it.}
    % Short version \Comment{\textbf{Note:} An edge added to $S$ is never
    % removed from it.}
    \EndIf
    \EndIf
    \EndFor
    \State Return $M$.
    \EndFunction
  \end{algorithmic}
\end{algorithm}
The charging scheme, and most of the Lemmas remain the same as
in~\Cref{sec:2pimp2}. We only prove the differences in this Section.
In the following Lemma, we bound the number of partially good edges in $M_0$
that are charged to one good edge.
\begin{lem}\label{lem4:2pimp3}
  At most $2\lambdaU-2$ partially good edges in $M_0$ are charged to one good
  edge in $M_0$. 
\end{lem}
\begin{proof}
  Suppose $uv\in M_0$ was augmented by edges $xu$ and $vy$ such that $xu$
  arrived before $vy$, then $xu \in S$.  Now $|N_S(x)|\le \lambdaU$, and
  $|N_S(y)| \le \lambdaU-1$. Since $xu \in S$, we have
  $|N_S(x)\setminus \{u\}| \le \lambdaU - 1$.  Let
  $B := (N_S(x)\setminus\{u\}) \cup N_S(y)$, then $|B| \le 2\lambdaU - 2$.  Now,
  the set of partially good edges that are charged to $uv$ is a subset of
  $M_0(B)$. Observing that $|M_0(B)| \le |B| \le 2\lambdaU -2$ finishes the
  proof.
\end{proof}

The following lemma gives a lower bound on the size of matching after one call
to \textproc{Improve-Matching}$()$.
\begin{lem}\label{eq:gbound3}
 Let $|M_0| = (1/2+\advntg)|M^*|$ and
  $M = \textproc{Improve-Matching}(M_0, \lambdaU, \lambdaM)$, then
  \[
    |M| \ge \left(\frac{1}{2} + \frac{\lambdaU-\lambdaM}{2\lambdaU(2\lambdaU-1)}
      +
      \left(1-\frac{3\lambdaU+\lambdaM}{\lambdaU(2\lambdaU-1)}\right)
      \advntg\right)|M^*|.  
  \]
\end{lem}
\begin{proof}
  By~\eqref{eq:bndgpg} and~\Cref{lem4:2pimp3}, the total number of
  augmentations during the second pass is at least
\begin{align*}
  \frac{1}{(2\lambdaU-1)} \left( \frac{\lambdaU-\lambdaM}{2\lambdaU}
  -\left(\frac{3\lambdaU+\lambdaM}{\lambdaU}\right)\advntg\right)|M^*|
  =\left(\frac{\lambdaU-\lambdaM}{2\lambdaU(2\lambdaU-1)}  
  -\left(\frac{3\lambdaU+\lambdaM}{\lambdaU(2\lambdaU-1)}\right)
  \advntg\right)|M^*|\,.   
\end{align*}
 
Hence, we get the following bound on the size of the output matching $M$:
\begin{align*}
  |M|&\geq |M_0| +\left(\frac{\lambdaU-\lambdaM}{2\lambdaU(2\lambdaU-1)}  
       -\frac{3\lambdaU+\lambdaM}{\lambdaU(2\lambdaU-1)}\advntg\right)|M^*|\\ 
     &=\left(\frac{1}{2} + \frac{\lambdaU-\lambdaM}{2\lambdaU(2\lambdaU-1)} +
       \left(1
       -\frac{3\lambdaU+\lambdaM}{\lambdaU(2\lambdaU-1)}\right)
       \advntg\right)|M^*| 
     && \text{because $|M_0| = (1/2 + \advntg)|M^*|$ }\,.
        \qedhere
\end{align*}
\end{proof}
We get the approximation ratios claimed in ~\Cref{tab:1} using the following theorem.
\begin{theorem}
  \label{thm:2pimp3}
  \Cref{alg:2pimp3} uses two passes and has an approximation ratio of
  $1/2 + 1/12.86$ for tri\-angle-free graphs and an approximation ratio
  of $1/2 + 1/28$ for general graphs for maximum matching.
\end{theorem}
\begin{proof}
  By~\Cref{eq:gbound3}, after the second pass, for triangle-free graphs, the
  output size $|M|\ge (1/2 + 1/12 -\advntg/6)|M^*|$ when $\lambdaU=2$ and
  $\lambdaM=1$, and the output size $|M|\ge (1/2 + 1/15 +\advntg/3)|M^*|$ when
  $\lambdaU=3$ and $\lambdaM=1$. The best of these two are output to get the
  required ratio.

  By~\Cref{eq:gbound3}, after the second pass, for general graphs, the output
  size
  $$|M|\ge \left(\frac{1}{2}
    +\frac{\lambdaU-\lambdaM}{2\lambdaU(2\lambdaU-1)}\right)|M^*|\,;$$
  see~Observation~\ref{note1:2pimp2}.  We use $\lambdaU=4$ and $\lambdaM=2$ to
  get the claimed approximation ratio.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_twopass"
%%% End:

